Technical Report: Modeling Average False Positive Rates of Recycling Bloom Filters

Bloom Filters are a space-efficient data structure used for the testing of membership in a set that errs only in the False Positive direction. However, the standard analysis that measures this False Positive rate provides a form of worst case bound that is both overly conservative for the majority of network applications that utilize Bloom Filters, and reduces accuracy by not taking into account the actual state (number of bits set) of the Bloom Filter after each arrival. In this paper, we more accurately characterize the False Positive dynamics of Bloom Filters as they are commonly used in networking applications. In particular, network applications often utilize a Bloom Filter that "recycles": it repeatedly fills, and upon reaching a certain level of saturation, empties and fills again. In this context, it makes more sense to evaluate performance using the average False Positive rate instead of the worst case bound. We show how to efficiently compute the average False Positive rate of recycling Bloom Filter variants via renewal and Markov models. We apply our models to both the standard Bloom Filter and a "two-phase" variant, verify the accuracy of our model with simulations, and find that the previous analysis' worst-case formulation leads to up to a 30\% reduction in the efficiency of Bloom Filter when applied in network applications, while two-phase overhead diminishes as the needed False Positive rate is tightened.

==> Repeat-text-removed.tex <==
\subsection{Repeat Messages}

BFs are only of use in environments where the process of arriving messages is a mix of new and repeat messages.  The traditional analysis that computes a worst case bound (i.e., (\ref{eq:wikiform})) need only evaluate new messages (repeats are true positives and hence have no false positive rate).  However, an average false positive rate can be described where repeats are excluded or included.  More formally, let $M(t)$ be the total number of messages to arrive by time $t$, where $N(t)$ of these messages are new ($M(t) - N(t)$ are repeats), and let $F(t)$ be the number of false positives during this time interval.  Then we can define the average false positive rate as either $\lim_{t \rightarrow \infty} F(t) / M(t)$ which includes repeat arrivals, or as $\lim_{t \rightarrow \infty} F(t) / N(t)$ which excludes new arrivals.

Our analyses below assume that the "newness" of a message is a Bernoulli process with probability $1 - p_r$, i.e., upon each message arrival, a biased coin is flipped and with probability $p_r$, the messages is a repeat, does not set any bits in the BF, and is classified by the BF as a repeat (true positive).  With probability $1-p_r$, the message is new, selects $k$ of $M$ bits in the BF, and sets those not already set.  If no new bits are set, the BF incorrectly classifies the message as a repeat (false positive).  Note that any formula that computes the average false positive rate of over all messages (i.e., the $\lim_{t \rightarrow \infty} F(t) / M(t)$) can be applied to compute the alternate new-only false positive rate (i.e., the $\lim_{t \rightarrow \infty} F(t) / N(t)$) by setting $p_r = 0$.


\subsection{Repeat arrivals}

Both (\ref{eq:wikiform}) and our previous Markov Model consider only the arrival of new messages, i.e., repeat messages do not occur.  Of course, any real application that utilizes BF does so to distinguish repeat from new arrivals.  We conclude this section by considering how new arrivals affect false positive rates of these differing modeling approaches.

We assume that each arrival is a repeat message (previously hashed into the BF) with probability $\pr$, and make an assumption that often holds in practice the process describing these arrivals is Bernoulli (i.e., flipping a $\pr$-biased coin to determine whether the next arrival is a repeat).  When the message is a repeat, since it has already hashed into the BF, no new bits are set, and the BF (correctly) reports the message is a repeat.

Modifying the Markov Model to account for new arrivals is straightforward.  In each state, we construct a new self-loop with probability $\pr$ to account for a new arrival.  This self loop differs from the previous self-loop in that it does not trigger a false positive event.  The remaining transitions are "thinned" by $1-\pr$ (i.e., a previous trransition of probability $q$ is now $q (1-\pr)$.

Note the above formulation assumes that only the first arrival of a message should be marked as new.  A subtle distinction might be made for certain applications where if the first time a message arrives it is counted as a false positive, then each successive repeat should also be counted as a false positive \dan{need to give a good app example here: akamai? would never cache a request that was f.p. on initial arrival.} \loqman{This phenomenon manifests in situations where the Bloom filter is employed as an intermediary to instigate actions on other segments of the systems. To illustrate this, we utilize an example outlined in Akamai \cite{maggs2015algorithmic}. Here, a Bloom filter is used to summarize the content hosted on a CDN server. In this case, a false positive indicates that an element appears to be present in the cache when, in reality, it is not. Every instance of an incorrectly forwarded request to the cache incurs a negligible overhead in performance for the end user. However, for popular elements, such instances accumulate and could lead to an aggregate performance decrease that is meaningful from Akamai's perspective. While the exact ways Akamai's caching systems handle those scenarios are unknown, this example demonstrates how a single false positive can instigate a cascade of effects that negatively affect other parts of the systems.}. Precise modeling of this \loqman{updated} false positive rate in a tractable manner is difficult because it depends on both the history of messages whose first arrival was a false positive and the respective arrival rates of different repeat messages.  However, this alternate definition of false positive rate can be bounded.  

We present two upper bounds: a looser (easy to see) bound and a tighter upper bound we have proven but whose proof is omitted due to lack of space: instead we sketch the idea behind the proof.  The looser upper bound simply assumes that every repeat arrival is considered a false positive (i.e., the self-loop with probability $\pr$ is treated as a false positive).  Since many first arrivals are unlikely to be false positives, this is a very loose upper bound.   It turns out that the original formulation (prior to introducing the repeat messages) is a much tighter upper bound.  The intuition behind the proof is based on the observation that repeat messages retain the false positive rate based on the order in the sequence with which they arrived to the BF.  Earlier messages have lower false positive likelihoods, so repeats, when sampled from earlier messages, retain this lower rate, bringing down the overall false positive rate in comparison to a process that does not have new arrivals.\dan{maybe we can share the pdf of the proof anonymously}.

\subsection{A lower bound on an $n$-insert average false positive rate}
\dan{dan to fill in}
